ResDTA: Predicting Drug-Target Binding Affinity Using Residual Skip Connections

The discovery of novel drug target (DT) interactions is an important step in the drug development process. The majority of computer techniques for predicting DT interactions have focused on binary classification, with the goal of determining whether or not a DT pair interacts. Protein ligand interactions, on the other hand, assume a continuous range of binding strength values, also known as binding affinity, and forecasting this value remains a difficulty. As the amount of affinity data in DT knowledge-bases grows, advanced learning techniques such as deep learning architectures can be used to predict binding affinities. In this paper, we present a deep-learning-based methodology for predicting DT binding affinities using just sequencing information from both targets and drugs. The results show that the proposed deep learning-based model that uses the 1D representations of targets and drugs is an effective approach for drug target binding affinity prediction and it does not require additional chemical domain knowledge to work with. The model in which high-level representations of a drug and a target are constructed via CNNs that uses residual skip connections and also with an additional stream to create a high-level combined representation of the drug-target pair achieved the best Concordance Index (CI) performance in one of the largest benchmark datasets, outperforming the recent state-of-the-art method AttentionDTA and many other machine-learning and deep-learning based baseline methods for DT binding affinity prediction that uses the 1D representations of targets and drugs.

==> inputs/abstract.tex <==
% Write theis abstract here as LaTeX text

The discovery of novel drug–target (DT) interactions is an important step in the drug development process. The majority of computer techniques for predicting DT interactions have focused on binary classification, with the goal of determining whether or not a DT pair interacts. Protein–ligand interactions, on the other hand, assume a continuous range of binding strength values, also known as binding affinity, and forecasting this value remains a difficulty. As the amount of affinity data in DT knowledge-bases grows, advanced learning techniques such as deep learning architectures can be used to predict binding affinities. In this paper, we present a deep-learning-based methodology for predicting DT binding affinities using just sequencing information from both targets and drugs. The results show that the proposed deep learning-based model that uses the 1D representations of targets and drugs is an effective approach for drug target binding affinity prediction and it does not require additional chemical domain knowledge to work with. The model in which high-level representations of a drug and a target are constructed via CNNs that uses residual skip connections and also with an additional stream to create a high-level combined representation of the drug-target pair achieved the best Concordance Index (CI) ~\cite{gonen2005concordance} performance in one of the largest benchmark datasets ~\cite{KIBA},
outperforming the recent state-of-the-art method AttentionDTA~\cite{attentiondta} and many other machine-learning~\cite{simboost, kronrls} and deep-learning~\cite{deepdta, mtdti, deepcpi, widedta, gansdta} based baseline methods for DT binding affinity prediction that uses the 1D representations of targets and drugs.




\endinput

==> inputs/acknowledgement.tex <==
% Write the acknowledgement text here as LaTeX text

I would like to thank Almighty as I have been able to successfully complete my thesis work.\\

I am indebted to my supervisor, Professor Dr. Md. Aynal Haque, whose expertise was invaluable in formulating the research questions and methodology. I would like to thank him for his guidance, assistance and patience throughout this research. Without his support and encouragement, it would not have been possible to complete the research work. His insightful feedback pushed me to sharpen my thinking and brought this work to a higher level. I am very lucky that I have got the opportunity to work under his supervision. I would also like to thank my senior Udoy Kamal and friend Proteeti Ghosh to constantly support me throughout the thesis and motivated me a lot.


\endinput
